Learning to Represent Patches

Patch representation is crucial in automating various software engineering tasks, like determining patch accuracy or summarizing code changes. While recent research has employed deep learning for patch representation, focusing on token sequences or Abstract Syntax Trees (ASTs), they often miss the change's semantic intent and the context of modified lines. To bridge this gap, we introduce a novel method, Patcherizer. It delves into the intentions of context and structure, merging the surrounding code context with two innovative representations. These capture the intention in code changes and the intention in AST structural modifications pre and post-patch. This holistic representation aptly captures a patch's underlying intentions. Patcherizer employs graph convolutional neural networks for structural intention graph representation and transformers for intention sequence representation. We evaluated Patcherizer's embeddings' versatility in three areas: (1) Patch description generation, (2) Patch accuracy prediction, and (3) Patch intention identification. Our experiments demonstrate the representation's efficacy across all tasks, outperforming state-of-the-art methods. For example, in patch description generation, Patcherizer excels, showing an average boost of 19.39% in BLEU, 8.71% in ROUGE-L, and 34.03% in METEOR scores.

==> 2.PrelimaryStudy.tex <==
% % \section{Running Example}
% \daniel{to come}

==> 4.MotivationExample.tex <==
\section{Motivation}
\tb{Do not touch motivation. I will delete it entirely by moving some text directly in approach} \daniel{Thanks, I've update the Figure 1 as pipeline, figure 2 as $Diff\_SEQ$ and figure 3 as $Diff\_AST$, so that it is in the right order as shown in the experiment and introduction. }
\subsection{Why transformer?}
Transformer architecture is demonstrated to have advantage in processing OOV problem and have strong transferability with pre-train and fine-tune strategy in NLP field.

\noindent
\textbf{OOV problem}
Compared with other NMT approaches, transformer-based methods (such as BERT \cite{devlin2018bert, sanh2019distilbert}) employs byte-pair-encoding (BPE \cite{shibata1999byte}) as its tokenizer, as a result, transformer-based methods have advantages to process OOV problem \cite{DBLP:journals/corr/SeeLM17}.

% \noindent
% \textbf{Long-text problem} strong in long text ontextual semantic extraction. The remarkable success of the transformer-based model in NLP has driven the development 

\noindent
\textbf{Strong Transferability} Transfer Learning has two steps, pre-training and fine-tuning. The first users the self-supervised method to predict the MASK data, and the latter fine-tunes the models on supervised tasks using labeled datasets. Transformer-based models has obtained remarkable success across many fields (\eg NLP, CV) with pre-trained and fine-tuned steps. Thus, for better inference in downstream tasks, we pretrain the parameters of transformer part in our \tool on a big java dataset for downstream tasks. 

\subsection{Why Contextual Information?}
As introduced in previous works \cite{jiang2017automatically,xu2019commit,yin2018learning}
Contextual text provides basic information for patches (\ie function names)

\subsection{Why Sequence Diff Embedding?}
Normally, as shown in Figure \ref{fig:java0}, patches contains two parts: contextual texts and modified lines, \ie plus lines and minus lines. Various works \cite{DBLP:journals/corr/abs-1911-11690,xu2019commit,hoang2020cc2vec} demonstrate that sequence diff (\ie modified lines) matter to generating description for the patches. We conduct an experiment to verify the effect of sequence diff for patch description generation on a selected a 2.2k dataset. The result in Table \ref{tab:seqdiff} indicates that `only SEQ diff' performs better than full dataset in most BLEU scores in GRU encoder-decoder. Specially, in a real case shown in Figure \ref{fig:java0}, GRU translator with only SEQ diff can generate the correct description for the patch while GRU translator failed in prediction with all patch information. The possible reason maybe that the whole patch is too long to the GRU translator.

% \begin{table*}[]
%     \centering
    
%     \caption{Patch description generation: comparison between full dataset and dataset with only sequential diffs or AST diffs. (All dataset support java compile. SEQ is short for sequence and AST is short for Abstract Syntax Tree.)}
%     \begin{tabular}{c|c|c|c|c|c}
%     \hline
%     \multicolumn{6}{c}{Baseline: GRU Encoder + GRU Decoder}\\
%     \hline\hline
%     BLEUs& BLEU-AVG& BLEU-1 & BLEU-2 & BLEU-3 & BLEU-4\\
%     \hline  
%     whole patch SEQ&18.51&30.7&18.5&15.5&14.6\\
%     \hline
%     only diff SEQ&19.07&30.0&19.0&16.7&16.5 \\
%     \hline
%     only diff AST&20.8&31.9&21.6&17.4&17.7\\
%     \hline
%     diff SEQ\&diff AST&\cellcolor{black!25}22.4&\cellcolor{black!25}32.7&\cellcolor{black!25}24.5&\cellcolor{black!25}17.9&\cellcolor{black!25}18.3\\
%     % \hline \hline
%     % ground truth& \multicolumn{5}{c}{A} \\
%     % \hline
%     % full dataset& \multicolumn{5}{c}{B} \\
%     % \hline
%     % only sequence diff& \multicolumn{5}{c}{C} \\
%     % \hline
%     % only AST diff& \multicolumn{5}{c}{C} \\
%     \hline
%     \end{tabular}   
%     \begin{tabular}{c|c}
%     \hline \multicolumn{2}{c}{Transformer (full dataset)} \\
%     \hline BLEU-AVG & 8.84 \\
%     \hline BLEU-1 & 21.1 \\
%     \hline BLEU-2 & 15.2 \\
%     \hline BLEU-3 & 14.9 \\
%     \hline BLEU-4 & 17.1\\
%     \end{tabular}
%     \label{tab:seqdiff}
% \end{table*}

\subsection{Why AST Diff Embedding?}
Prior works \cite{zhang2019novel,mou2016convolutional,white2016deep,wei2017supervised} provide the strong evidence that syntactic knowledge contributes more in modeling source code and can obtain better representation than traditional token-based methods. These approaches combine AST and Recursive Neural Network (RvNN) \cite{white2016deep}, Tree-based CNN \cite{mou2016convolutional} or Tree-LSTM \cite{wei2017supervised} to capture both the lexical (\ie the leaf nodes of ASTs such as identifiers) and syntactical (\ie the non-leaf nodes of ASTs like the grammar construct WhileStatement) information. Such AST-based neural models are effective, yet they have two major limitations. First, similar with long texts problem in NLP, these tree-based neural models are vulnerable to the gradient vanishing problem that the gradient becomes vanisingly small during training, especially when the tree is very large and deep \cite{bengio1994learning,hochreiter1998vanishing,le2016quantifying}. Second, using ST-trees as input or view ASTs as full binary trees disable the model to get the global structure of source code and even make the ASTs impossible for graph embedding because ASTs diff the size to each other. 

In order to address the limitations of the above AST-based neural works, our solution is to build a static graph based on all AST sub-graphs on training data, then align sub-graphs to the same size of static graph, and finally conduct graph convolutional embeddings to generate final AST embeddings.

==> Background.tex <==
\section{Background}\label{sec:background}

==> Novelty.tex <==
\section{Novelty Declaration}

\begin{figure*}[htbp!]  

	\centering
    \subfigure[An example of patch and description]{
		\includegraphics[width=7cm]{pictures/patchexample.pdf}
		\label{Fig:patchexample}
	}
	\quad
	\subfigure[Main component in CACHE]{
		\includegraphics[width=8cm]{pictures/CACHE.pdf}
		\label{Fig:cacheexample}
	}
	\quad
	\subfigure[Main component in FIRA]{
		\includegraphics[width=8cm]{pictures/firaexample.pdf}
		\label{Fig:firaexample}
		%\caption{FIRA}
	}
	\quad
	\subfigure[Simple pipeline of \textbf{AST diff} calculation in \tool]{
		\includegraphics[width=8cm]{pictures/patcherizerexample.pdf}
		\label{Fig:patchastexample}
	}
	\caption{Comparison with AST-based Approaches}
	\label{Fig:motivate_example}	
\end{figure*}

Previous Literature investigates patch embedding with various techniques. Given a code change, these techniques first represent the old-version and new version code with specific formats, such as sequences of tokens or paths of abstract syntax tree (AST), and implement patch downstream tasks based on the representations via different strategies, such as fusion of context-based~ \cite{hoang2020cc2vec,xu2019commit,xu2022combining}, and AST-based~\cite{dong2022fira,liu2020atom,lin2022context}. As our \tool are based on both Seq Diff (not Seq) and AST Diff (not AST), in this section, we mainly focus on declaring our novelty against previous works on both sequence and structure.

\textbf{Novelty on sequential part.} As shown by the example in Figure~\ref{Fig:patchexample}, we can observe that both contextual information and code changes are highly relevant to developer-written patch messages. The developer make change operation (\ie change getMaxEnergyReceived to getActivationEnergy in powerRequest function). However, existing techniques cannot always notice such edit operations, since their code change representations put old version and new-version code together without explicitly highlighting the difference. Therefore, they have to compare old-version and new-version code and then infer the edit operations by combining various calculation between code changes (\ie add, minus, time, cosine, concatenate, etc). In our \tool, we design Diff-SEQ module (Sec~\ref{seq-diff}) for highlighting the difference. Different from illogical addition, subtraction, multiplication, and division splicing of added line and removed lines in previous works~\cite{xu2019commit,hoang2020cc2vec,nie2021coregen}, we design cross-attention and cross-resnet functions in Diff-SEQ for injecting contextual semantics into the semantic of code changes, and calculate the intention among changed lines, which is introduced in detail in Sec~\ref{seq-diff}.% at the sequence level by comparing the added line with the removed line (this part will be introduced in detail in chapter XXX); 
% CoDiSum~\cite{xu2019commit} is one state-of-the-art token-based approaches~\cite{xu2019commit,hoang2020cc2vec,nie2021coregen} in patch message generation task. 


\textbf{Novelty on structural part.} CACHE~\cite{lin2022context}~(Figure~\ref{Fig:cacheexample}) and FIRA~\cite{dong2022fira}~\ref{Fig:firaexample} are two representative AST-based approaches for patch representation. CACHE mainly focuses on combining AST context information, removed AST branches, and added AST branches for patch representation. The motivation of CACHE is that the AST context has strong contextual semantics. However, according to our statistics analysis, compared with sequential codes, 97.33\% tokens output from AST compile system, and these most of these tokens are unrelated with patch, such as variables (\ie sub\_type, ReferenceType, etc.) with a large number of null values. Thus, only enhancing the semantics of added AST branches or removed AST branches by using AST context will inject much noisy information into the patch representation. In fact, AST-based models (\ie FIRA~\cite{dong2022fira}) have proved that only using AST is not enough for representing the semantic of patch. The biggest reason maybe that 97.33\% tokens of AST are not related to the patch.

Another representative AST-based approach, FIRA~\ref{Fig:firaexample}, mainly focuses on the editing AST. Added node will be linked to a node named ``ADD" neighbor the removed node will linked to a node named ``REMOVE'', and the unchanged nodes are connected with the ``MATCH" edge. After that, FIRA obtains edition graph. At the same time, the code before patching and the code after patching are connected into a one-line graph according following the rule that neighboring tokens are connected with an edge. Finally, the edition graph and one-line graph are combined to generate the final graph by merging common nodes. However, as described in ablations study in FIRA~\cite{dong2022fira}, the main contribution of FIRA comes from the one-line graph, which is actually sequential part. Furthermore, FIRA recognizes the intention of the patch by adding semantics such as ``ADD'' and ``REMOVE'' into the AST by adding nodes. Due to that large amount of noise in the AST Tokens and GCNs are calculated based on tokens and topological structures, which prevents the semantics of edge nodes such as add and remove from appearing in the graph representation of the entire graph. Thus, FIRA's AST part is not as effective as one-line graph since FIRA represents patch by embedding the entire graph. %By randomly sampling the data in FIRA multiple times, the average entry and exit degrees of the remove and add nodes formed by each patch are much lower than the average entry and exit degrees of other nodes in the graph.

In our \tool, we design Diff-AST module (Sec~\ref{seq-diff}) for highlighting the semantic of differential nodes between before-patching AST and after-patching AST. Different from CACHE~\cite{lin2022context} and FIRA~\cite{dong2022fira}, Diff-AST module leverages removed node and added node embedding (instead of whole graph representation) as AST representation . Embeddings of added or removed AST branches not only contains semantics from contextual AST but also retains patch intention in structure, which will be discussed in Sec~\ref{sec:graph_extractor}.

%the context semantics of AST, but also removes AST and added AST due to the self-loop mechanism in GCN The representation of the whole graph has more intent recognition capabilities than the whole graph representation (this part will be introduced in detail in Chapter XX); 

\textbf{Novelty in combining Diff-SEQ and Diff-AST modules.} As shown in Sec~\ref{sec:assembling}, we merge semantics from Diff-SEQ and Diff-AST modules by $\mathcal{Add}$ aggregation function.%We design corss resnet tothe fusion module cleverly integrates Seq diff and AST diff through cross resnet attention, and enhances the context of AST diff from the sequential level semantics (addressing the flaws in Wang's work), while enhancing the structured semantic information of seq diff.


In summary, the novelty of \tool can be summarized as threefold:
\begin{itemize}
    \item Compared with previous token-based techniques~\cite{hoang2020cc2vec,xu2019commit,xu2022combining}, our \tool proposes Diff-SEQ module for highlighting the difference in patch. 
    \item Compared with previous AST-based techniques~\cite{dong2022fira,liu2020atom,lin2022context}, our \tool proposes Diff-AST module for highlighting the patch intention because we use differential node embeddings (instead of whole graph embeddings) out of GCN operation as AST Diff embeddings.
    \item We leverages $\mathcal{Add}$ aggregation function to merge sequential and structural semantics as the final patch representation.
\end{itemize}
% Compare we have solved the semantic extraction of patches at the sequentially level more logically by designing the Seq diff module; by designing the AST diff module, we have more accurately expressed the changes in the AST structure before and after the patch. Semantic changes; By designing a semantic fusion model, the Patcherizer's ability to extract the semantics of the structural and sequential changes in the code before and after the patch is enhanced.




% Although achieving promising performance, the effectiveness of previous techniques has been restricted by their coarse-grained code change representations. For example, given an expression ``a=1;'' modified into ``a-=1'', context-based techniques~\cite{hoang2020cc2vec,lin2022context,xu2019commit} represent such code changes by various concatenating both expressions into one combined tokens (i.e., ``=1; -=1; =1--=1; =1+-=1; =1*-=1; =1/-=1'', which doesn't make any sense to do ``*'' or ``/'' between old and new version codes. For previous AST-based codes, they involve whole AST into consideration that will lead dirty words injection to the model because AST compiler will produce plenty of rule words as the output.

% Different from previous context-based code changes and AST-based techniques, \tool focus on AST diffs and fusion between AST diffs and SEQ diffs. \tool does not involve dirty information from AST compiler. Moreover, \tool make it easy to recognize the intention of the patch in structurally and sequentially. For example, ``a+b'' and ``b+a''  has no difference in AST but they means change order in the difference in sequence.

% As the example above, AST diff module can recognize the intention of the patch is to do changes from ``=1'' to ``-=1''.

==> backup-intro.tex <==
\section{Introduction}\label{sec:intro}
% Guidance:
% \begin{itemize}
%     \item \textcolor{red}{what is patch}
%     \item \textcolor{red}{why patch embedding is important and what application of patch}
%     \item \textcolor{red}{how about other previous works on patch presentation: downstream tasks, advantages addressed, and left shortcomings and challenges}
%     \item \textcolor{red}{What is our approach}
%     \item \textcolor{red}{what is our contribution}
% \end{itemize}

A software patch represents the source code differences between two software versions. It has a dual role: on the one hand, it serves as a formal summary of the code changes that a developer intends to make on a code base; on the other hand, it is used as the main input specification for automating software evolution. Patches are thus a key artefact that is pervasive across software development lifecycle. In recent years, building on empirical findings on the repetitiveness of code changes,  several approaches have built machine learning models based on patch datasets to automate various software engineering tasks such as patch description generation~\cite{linares2015changescribe,buse2010automatically,cortes2014automatically,jiang2017automatically,xu2019commit,liu2019generating,liu2018neural,liu2020atom}, code completion~\cite{svyatkovskiy2019pythia,liu2020multi,liu2020self,ciniselli2021empirical,pian2022metatptrans}, patch correctness assessment \cite{tian2022change}, and just-in-time defect prediction \cite{hoang2019deepjit,kamei2016studying}.

In the aforementioned research directions, devising a patch representation that is suitable for the addressed task is a major challenge. 
Many initial works proposed to manually craft a set of features to represent a patch~\cite{kamei2016studying,kamei2012large}. 
More recently, with the successful application of deep learning methods for representing texts, signals and images in various fields~\cite{devlin2018bert,jiang2021cure,tian2022change,niemeyer2021giraffe,qin2021co,li2021attention,tang2021moto,pian2022metatptrans}, software engineering researchers have considered the development of deep learning models to represent code and code changes~\cite{hoang2020cc2vec,feng2020codebert,nie2021coregen}. 
These approaches generally consider code, and other code-like texts such as patches, as pure sequential text and thus employ natural language processing methods to extract code syntax semantics. 
For code changes, the differences in code token sequences (represented by {\tt +} and {\tt -} lines) are however not sufficient to represent the full semantics of the changes (e.g., what code behaviour is affected). 
To capture code behaviour change, it is essential to capture structural information differences. 
Recent works~\cite{cabrera2021commit2vec,brody2020structural}, such as commit2vec, have attempted to account for Abstract Syntax Tree (AST) information. 
Unfortunately, these approaches miss exploring explicitly the AST differences in the code diff itself. Furthermore, it is noteworthy that a few prior works~\cite{see2017get,xu2019commit}  on  code change representation learning have attempted to address the out-of-vocabulary (OOV) problem by employing some copy mechanism, which unfortunately required two training strategies for a single model. 
More recent works~\cite{nie2021coregen,feng2020codebert,wang2021codet5,elnaggar2021codetrans} have demonstrated that Transformers architecture~\cite{devlin2018bert,DBLP:conf/dasfaa/WangTZLH22} and byte-pair-encoding (BPE)~\cite{shibata1999byte} can effectively address this problem. 
Finally, we note that various approaches of patch representation learning approaches in recent years have focused on specific tasks (e.g., FIRA~\cite{dong2022fira}, CoDiSum~\cite{xu2019commit}), CoreGen~\cite{nie2021coregen}, etc.). 
The incumbent state of the art that aims for general representations is CC2Vec\cite{hoang2020cc2vec}.
However, its training is still task-driven; it is further focused on sequential differences and thus generally fail to identify similar structural changes, which is important in code semantics.


{\bf This paper.} We propose \tool, a graph-based approach for representation learning of code changes. \tool copes with the shortcomings of prior approaches by attempting to combine several information modalities (i.e., code context, code sequence differences, code AST differences) into a single graph representation that is fed to a Transformer architecture. 
\tool can be used by researchers and practitioners as a pre-trained encoder-decoder model for patch embedding, which can be applied to a variety of tasks including patch description generation, patch correctness validation for program repair or defect-prediction. 


%Despite the comparative successes of deep leaning methods in representing patches, all of these studies suffer from the following limitations: out-of-vocabulary (OOV) problem, long-text problem. To address the OOV problem, \cite{see2017get,xu2019commit} employ a kind of copy mechanism, but it will make the model incongruent because there will be two training strategies in one model. To address this challenge,  employ transformer architecture and byte-pair-encoding (BPE) . In this work, we follow them and employ transformer and BPE to tokenize and embed code modifications and code context.

%Patches, used to be known as source code changes, are ubiquitous in code commits, feature pull requests, bug fixing, etc. Usually, there are two main parts in a patch\tian{or we say, A generalized patch typically contains two parts}: patch description and a snipet of code changes. The patch description is normally written in natural language by the developers, which is used to describe the intention of the patch. The source code changes include plus lines, minus lines and their contextual source codes across one or multiple files. Prior studies have confirmed that patches are repetitive in software engineering problems, such as patch description generation \cite{linares2015changescribe,buse2010automatically,cortes2014automatically,jiang2017automatically,xu2019commit,liu2019generating,liu2018neural,liu2020atom}, code completion \cite{svyatkovskiy2019pythia,liu2020multi,liu2020self,ciniselli2021empirical,pian2022metatptrans}, code summary generation \cite{ahmad2020transformer,leclair2020improved,zhu2019automatic,zhang2020retrieval,wan2018improving}, code comment generation \cite{hu2018deep,hu2020deep,li2022setransformer,li2021secnn}, just-in-time defect prediction \cite{hoang2019deepjit,kamei2016studying},etc. %The most popular approaches for these tasks are deep learning methods.
% \tian{the importance of patch embedding is not explicitly describe. Like, the learning representation of patch is leveraged to predict patch correctness. and so on.}
% Exploring patches to solve software engineering problems above requires good representations of patches. Most prior traditional works involve manually crafting a set of features to represent a patch and using these features for further processing \cite{kamei2016studying,kamei2012large}.  Recently, deep learning methods are playing an increasing important role on representing texts, signals, and images in various fields\tian{cite references}. At the same time, it grows fast that interest emerged in the research community to explore similar methods to the analysis of patches. Some deep learning methods are widely used to represent code-like texts, such patch, commits \cite{hoang2020cc2vec,feng2020codebert,nie2021coregen}. These approaches take patches and code-like texts as pure sequential texts and employ natural language processing methods to extract code syntax semantics with feature extraction calculation among plus and minus lines\tian{same as before}. As a result, deep learning methods succeed in representing patches and address part of tasks related to patches (e.g., commit description generation)\tian{redundant/duplicated sentence.}. 

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=1\linewidth]{pictures/ast_diff_example.pdf}
%     % \vspace{0.5mm}
%     \caption{A simple example of AST diff.}
%     \label{fig:astdiffexample}
% \end{figure}

%\tian{i don't get the meaning of this paragraph.}
%However, different from pure source codes, the key features of patches are the diff parts. Normally, pure source codes have two kinds of aspects for representing them: sequential syntax semantics and abstract syntax tree semantic. Similarly\tian{In the first sentence, you say "different from...", but then here you are talking about the "similarly,...". It's anti-logical.}, patches has two main semantic features: sequential diff part and AST diff part. Sequential diff part contains modified lines (plus lines and minus lines) and AST diff means the diff graph of before-patch codes and after-patch codes.


% \begin{lstlisting}[language=diff]
% public abstract class HardwareRenderer {
% public static boolean sSystemRendererDisabled = false ; 
% - public static boolean sUseRenderThread = true ; 
% + public static boolean sUseRenderThread = false ; 
% private boolean mEnabled ; 
% private boolean mRequested = true ; 
% }
% \end{lstlisting}


%\caption{description:annotate stacktrace only in " analyze stacktrace " and thread dump console}

% For example, these features can be extracted from the various names in the modified lines (plus lines and minus lines). Then, they employ these features as input into traditional machine learning classifier (e.g, Support Vector Machine, Random Forest, XGBOOST, etc.) for software engineering downstream tasks \cite{kamei2016studying,kirinuki2014hey,rahman2016correct,tian2012identifying}.

%Despite the comparative successes of deep leaning methods in representing patches, all of these studies suffer from the following limitations: out-of-vocabulary (OOV) problem, long-text problem. To address the OOV problem, \cite{see2017get,xu2019commit} employ a kind of copy mechanism, but it will make the model incongruent because there will be two training strategies in one model. To address this challenge, \cite{nie2021coregen,feng2020codebert,wang2021codet5,elnaggar2021codetrans} employ transformer architecture and byte-pair-encoding (BPE) \cite{shibata1999byte}. In this work, we follow them and employ transformer and BPE to tokenize and embed code modifications and code context.

%Apart from sequential semantics, the semantics of a patch also benefits from its syntax structural information. The semantic of a patch is also embedded in its abstract syntax trees (AST) \footnote{A patch can be processed as two source codes, one is before the changes and the other is after the changes. Both source codes have their AST, and we can extract structure information with these ASTs for a patch.}. Specially, \cite{cabrera2021commit2vec,brody2020structural} represent patches with syntactic structure information for commit2vec. However, these structural semantic mining from ASTs is still not enough to explore, For example, structural information of specific code changes is still unexplored because previous researches process ASTs in codes before and after a change, respectively, not the code diff itself.
%Towards building a gene
%Overall, we postulate that learning patch representations requires addressing three main challenges: \ding{182} Embed syntax semantic of contextual information of code changes in patches ;\ding{183} Enhancing sequential diffs (modified lines, normally refers to plus lines and minus lines) and fusing them with representations in \ding{182}; \ding{184} Enhancing structural AST diff in patch and aggregate with \ding{182} and \ding{183}.
% To address challenges above, in this work, we propose \tool, a pre-trained encoder-decoder model that considers both sequential semantic extraction and code diff structure semantic extraction.
% \textbf{For challenge \ding{182}}, our \tool builds on the transformer architecture that is well-applied in the NLP community \cite{sanh2019distilbert,devlin2018bert,DBLP:conf/dasfaa/WangTZLH22}. Prior research works \cite{xu2019commit,wang2021codet5,nie2021coregen} have demonstrated that transformer employs denoising sequence-to-sequence (Seq2Seq) pre-training and benefit both understanding and generation tasks in natural language. Furthermore, transformer-series approaches are enable to fix the out-of-vocabulary (OOV) problem that is common in other neural machine translaton (NMT) approaches. As we know, there exist plenty of UNK words (OOV problem) in source codes. Thus, we employ BPE tokenizer and transformer-based architecture in \tool. \textbf{For challenge \ding{183}}, we also employ transformer with BPE tokenizer as the semantic extractor of sequential diffs. Furthermore, as shown in Figure \ref{fig:patchformer}, we design a operation-wise and context-wise operator to make \tool sensitive about intentions of patches. \textbf{For challenge \ding{184}}, as shown in Figure \ref{fig:astdiff}, we propose a architecture of AST diff embedding calculator to get structural semantics for patches. Specially, firstly, we design a rule to rewrite the patch and generate codes before patch and codes after patch. Then, we generate use javalang \footnote{\url{https://github.com/c2nes/javalang}} to extract ASTs for rewritten codes and design a AST2Parser \footnote{\url{https://anonymous.4open.science/r/AST2Graph-41E2/README.md}} to transfer ASTs to graphs and visualization. Next, we merge all graphs into a static graph and align all graphs the size of the static graph. Finally, we conduct GCN embedding on these AST graphs to obtain AST diff embeddings.
Our contributions are as follows:

% Prior studies have confirmed that software patches are repetitive \cite{barr2014plastic}
Our contributions are as follows:
\begin{itemize}
    % \item [$\blacktriangleright$] We develop a rewritten tool for generating valid source codes from patches which can pass Java Compiler and finally we get a 2.2k-size dataset for patch description generation.
    \item [$\blacktriangleright$] Most existing datasets are provided with incomplete java patches (or diffs) which lead that we cannot extract AST from the code\_before\_patch and  code\_after\_patch. Therefore we develop a rewritten tool and finally obtain final 2.2k dataset which can pass the java compiler and generate ASTs for both code\_before\_patch and code\_after\_patch.
    \item [$\blacktriangleright$] To the best of our knowledge, we are the first to design a AST diff semantic extractor. Besides, we are the first to combine both sequence diff and structure diff for embedding patch for its downstream tasks.
    \item [$\blacktriangleright$] The experimental results indicates that both SEQ-diff and AST-diff in patches matter to the semantic of patches and our \tool outperform all the metric compared with other SOTAs.
\end{itemize}

==> exp/rq1.3.tex <==
\noindent
%\textbf{[Experiment Goal (RQ-1.3)]:}
%In this section, we compare our \tool with the same patch representation method CC2Vec \cite{hoang2020cc2vec} on the task of just-in-time (JIT) defect prediction to the identification of defective patches. JIT defect prediction tools are used to provide early feedback to software developers to optimize their effort for inspection~\cite{schutze2008introduction}. Following the previous approaches \cite{hoang2020cc2vec,zhang2015sensitivity}, we formulate JIT defect prediction as a binary classification task, in which, given a patch containing a code change and a log message, we label the patch with buggy or not.

% \noindent
% \textbf{[State-of-the-art Approach (RQ-1.3)]:} The state-of-the-art approach is CC2Vec, proposed by Hoang~\etal~\cite{hoang2020cc2vec}. CC2Vec learns distributed representations of code changes in the whole dataset \cite{mcintosh2018fix}. In JIT defect predict task, CC2Vec generates the embeddings of given patches and merges them with embeddings for the patch and corresponding log message from DeepJIT \cite{zhang2015sensitivity}. CC2Vec obtains good performance because of its fusion of code changes. However, CC2Vec ignores the contextual information because of its semantic fusion strategy, not including the contextual {\tt MASK} prediction so that CC2Vec is a highly task-relied method and poor in extracting contextual semantics and historic knowledge from the trained weight from other tasks.

\noindent
\textbf{[Experiment Design (RQ-1.3)]:} Following prior work~\cite{hoang2020cc2vec}, we integrate \tool with DeepJIT~\cite{zhang2015sensitivity}. Given one patch, we generate its embedding and concatenate the generated vector of the patch with the vector of the associated commit message and output the final new embedding vector. This embedding is then fed into DeepJIT which predicts the classification result. Unfortunately, the datasets (QT and OPENSTACK) are not parsable to retrieve ASTs. Therefore, we use a variant of \tool without the graph intention encoding (i.e., \tool$_{GraphIntention-}$).
%
We use 5-fold cross-validation for the evaluation. The metric to evaluate JIT defect prediction is {AUC}, and the relevant baseline is CC2Vec.

\noindent
\textbf{[Experiment Results (RQ-1.3)]:}
The classification performance are depicted in Table~\ref{tab:rq1.3}. \tool improves the AUC scores about 2 percentage points on both  the {\tt QT} and the {\tt OPENSTACK} datasets. Note that this performance improvement is achieved although \tool could not even embed structural differences in patches.
%Specially, \tool improve the AUC score on {\tt QT} 2.30\% compared with CC2Vec and 1.73\% on {\tt OPENSTACK}. This indicates that \tool is effective.


\input{table/rq1.3}

\find{{\bf \ding{45} Answer to RQ-1.3: }$\blacktriangleright$ 
The experimental results show that the embeddings produced by \tool$_{diff_{AST}-}$ are effective for the just-in-time defect prediction task. While those embeddings were initially obtained through a task-agnostic pre-training, they outperform the embeddings by CC2Vec, which were produced using the patch description information that is also leveraged in the defect prediction.
%to It even improves The experiment on JIT defect prediction indicates that compared with the state-of-the-art technique, \tool is more effective at learning representations of patches and \tool improves the AUC scores 1.73\% and 2.30\% on datasets {\tt QT} and {\tt OPENSTACK}, respectively.
$\blacktriangleleft$ }

==> exp/rq4.tex <==
\subsection{[RQ-4] Human Evaluation} 





==> exp/rq5.tex <==
\subsubsection{RQ-5} Impact of Parameters
\begin{table*}[]
    \label{tab:parameter}
    \caption{Performance of \tool with different sets of parameters on patch description generation (dataset\#2).}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
         Layer-2, Header-M& BLEU-1 Score &Layer-4, Header-M& BLEU-1 Score&Layer-6, Header-M& BLEU-1 Score \\
         \hline
         L2, H2 &  &L4, H2 & &L6, H2 &\\
         \hline
         L2, H4 &  &L4, H4 & &L6, H4 & \\
         \hline
         L2, H6 &  &L4, H6 & &L6, H6 & \\
         \hline
    \end{tabular}
\end{table*}

In this experiment, we select 3 values for layers and headers in the transformer for the patch description generation task. As a result, we have 9 pairs of layer-header parameters. The three values are: 2, 4, and 6, which are shown in Table~\ref{tab:parameter}.

==> table/exporg.tex <==
\begin{table}[H]
\caption{Overall information of experiment organization.}
\resizebox{0.6\linewidth}{!}{
\begin{tabular}{c|c|c|r}
\toprule
 \diagbox{{\bf Tasks}}{{\bf Datasets}} & {\bf \#1} & {\bf \#2} & {\bf \#3}  \\ 
\midrule
{\bf PDG} & \makecell[c]{\ding{52} } & \makecell[c]{\ding{52} }   & \makecell[c]{\ding{52}}\\ \hline
{\bf PV} &           &           & \ding{52}  \\ \hline
\end{tabular}}
\begin{tablenotes}
\item ``PDG" means patch description generation and ``PV" is patch validation.
\item ``\#'' means the number of dataset or task.
\item ``\ding{52}'' means pair of {\bf T\#?} and {\bf Dataset \#?}.
%\item ``\ding{52}[RQ-?]'' means the pair of \texttt{<}{\bf T\#?}, {\bf Dataset \#?}\texttt{>} and the pair is verified to answer the RQ-?.
\end{tablenotes}
\label{tb:expinfo}
\end{table}

==> table/rq1.3.tex <==
\begin{table}[!t]
    \centering
    \caption{AUC (\%) Results on JIT defect prediction on QT and OPENSTACK datasets.}
	\resizebox{0.6\linewidth}{!}
	{
 % \begin{tabular}{lp{1.5cm}cp{1.5cm}cp{1.5cm}}
\begin{tabular}{lrr}
    \toprule
      Model &  QT & OPENSTACK \\ 
     \midrule
     DeepJIT & 76.8 & 75.1 \\
    CC2Vec & 82.2 & 80.9\\ \cline{1-3}
    % \tool & 84.5 & 82.3 \\
     {\tool$_{diff_{AST}-}$} & 84.5 & 82.3 \\
     \bottomrule
    \end{tabular}
    }
    \label{tab:rq1.3}
\end{table}
